What Algorithms can Transformers Learn? A Study in Length Generalization

Large language models exhibit surprising emergent generalization properties, yet also struggle on many simple reasoning tasks such as arithmetic and parity. This raises the question of if and when Transformer models can learn the true algorithm for solving a task. We study the scope of Transformers' abilities in the specific setting of length generalization on algorithmic tasks. Here, we propose a unifying framework to understand when and how Transformers can exhibit strong length generalization on a given task. Specifically, we leverage RASP (Weiss et al., 2021) -- a programming language designed for the computational model of a Transformer -- and introduce the RASP-Generalization Conjecture: Transformers tend to length generalize on a task if the task can be solved by a short RASP program which works for all input lengths. This simple conjecture remarkably captures most known instances of length generalization on algorithmic tasks. Moreover, we leverage our insights to drastically improve generalization performance on traditionally hard tasks (such as parity and addition). On the theoretical side, we give a simple example where the "min-degree-interpolator" model of learning from Abbe et al. (2023) does not correctly predict Transformers' out-of-distribution behavior, but our conjecture does. Overall, our work provides a novel perspective on the mechanisms of compositional generalization and the algorithmic capabilities of Transformers.

==> gotu_app.tex <==
\pnote{UNUSED!!! scratch work only}


\clearpage
\section{GOTU}

Here we show an example setting where our RASP-based toy model of learning
is more predictive than the min-degree-interpolator model proposed in \citet{abbe2023generalization}.
Thus, we argue that for Transformer learning, it is more appropriate to use ``RASP-length'' 
rather than ``polynomial degree'' as the notion of complexity.

Specifically, we will show a setting where:
\begin{itemize}
    \item The min-degree-interpolator on the train set has degree $15$.
    On the unseen test set, this interpolator always predicts the constant $1$.
    \item There exists a 1 line RASP program which interpolates the train set.
    This program has polynomial degree $20$, and is not constant on the unseen test set.
    \item When a Transformer is trained on the train set, its
    predictions on the unseen test set agree almost perfectly with the above RASP program,
    but not with the min-degree-interpolator.
    That is, the trained Transformer behaves exactly like the short RASP program,
    and entirely unlike the min-degree-interpolator.
\end{itemize}

\paragraph{Setting}
The setting is as follows.
The ground truth function is the boolean AND of all $n=20$ input bits:
\[
f^*(x_1, x_2, \dots, x_{n}) = \bigwedge_{i \in [n]} x_i
\]
where $x_i \in \{0, 1\}$.

The train distribution is:
with probability $1/2$, $x$ is the all-ones vector ($x = 1^n$);
with probability $1/2$, $x$ is an all-ones vector with a single $0$ in a random location among the first 15 bits.
That is,
\[
x \sim (1^n - B(\nicefrac{1}{2})e_i); \quad i \sim \mathrm{Unif}[1, 15]
\]
where $e_i \in \{0, 1\}^n$ is the $i$th standard basis vector.
Note the ground-truth label $y = f^*(x)$ for this distribution is balanced.

The unseen test distribution is
identical to the train distribution, except the '0' is only among the last $5$ bits.
That is,
\[
x^{\textrm{(Unseen)}} \sim (1^n - B(\nicefrac{1}{2})e_i); \quad \textbf{$i \sim $ {Unif}[16, 20]}
\]

\paragraph{Min-Degree Interpolator}
The ground-truth function $f^*$ has polynomial degree $n=20$.\footnote{One may observe that
the boolean AND function has small \emph{sign-degree}, since it is a Linear Threshold Function.
Here we consider only the strict polynomial degree, following \citet{abbe2023generalization},
but it is an open question whether \citet{abbe2023generalization} can be extended
to more robust measures of degree.
}
The min-degree-interpolator, however, has degree at most $15$, since the following function interpolates:
\[
\widetilde{f}(x_1, x_2, \dots, x_{20}) = \bigwedge_{i \in \{1, 2, \dots, 15\}} x_i.
\]
Note $\widetilde{f}$ is simply the boolean AND of the first 15 coordinates.
In particular, the min-degree interpolator will not depend on the last $5$ input bits,
since they are always constant ($1$) in the train set.

On the other hand, there is clearly a one-line RASP program which implements the boolean AND on all 20 bits:
\verb|out = 1-kqv(x, fill(x, 0), fill(x, 1), equals)|

\paragraph{Experimental Results}

When a standard decoder-only Transformer is trained in the above setting,
it reaches 100\% test accuracy on the unseen test set.
That is, the trained Transformer agrees with $f^*$, the boolean AND over all 20 input bits,
which cannot be the case for the min-degree interpolator.
Note, this experimental result holds both
when ``packing the context'' and random shifting is used,
and when it is not.

\subsection{More formally}

We claim that the min-degree-interpolator in the above setting
does not depend on the last 5 coordinates. This follows from the below simple lemma,
which uses the same notion of ``degree profile'' as in GOTU \citet{abbe2023generalization}.

\begin{lemma}
Let $f: \{\pm 1\}^n \to \{\pm 1\}$
be a boolean function.
Suppose $f$ depends on its first coordinate; that is
suppose $\exists z \in \{\pm 1\}^{n-1}: ~~f(0 \circ z) \neq f(1 \circ z)$.
Then, restricting the first coordinate of $f$ to be $1$ strictly reduces its degree profile:
\[
\mathrm{DegP}(f\vert_{x_1 = 1}) < \mathrm{DegP}(f)
\]
\end{lemma}
\begin{proof}
(Sketch).
Consider the multilinear representation of $f$, and factor out terms containing $x_1$:
\begin{align}
f(x_1, \bar{x}) &= x_1 P(\bar{x}) + Q(\bar{x}) 
\end{align}
where $\bar{x}$ denotes $(x_2, x_3, \dots, x_n)$.
When restricted with $x_1=1$, we have
\begin{align}
f(x_1, \bar{x})\vert_{x_1 = 1} &= P(\bar{x}) + Q(\bar{x}) 
\end{align}
Now, because $f$ depends on $x_1$ by assumption, we must have $P \neq 0$.
Thus, comparing the above two, at least one monomial containing $x_1$
has reduced degree with the restriction. The conclusion follows.
\end{proof}


==> toymodel.tex <==
\section{Toy Model: Systematic Generalization via Marginal-matching}

In this section, we formalize our intuition from the counting task and present a simplified toy model of learning in which length-generalization provably occurs. While this toy model is clearly a simplification, we use it to develop a heuristic which often correctly predicts transformer length-generalization.





















\subsection{lifted marginals formulation}

\begin{assumption}[Minimal-Description-Length learning]
\label{conj:rasp}
There exists a \emph{complexity measure} on functions $\mu: \mathcal{F} \to \R_{\geq 0}$
such that the following holds.
On symbolic tasks defined by a distribution $\cD_f$ on prompt-completion pairs $(x, f(x))$,
the result of training a transformer on $\cD_f$
is equivalent to a minimal-complexity function that perfectly fits $f$.
That is,
\[
f^* \in \argmin_{g:~~ \mathrm{Loss}(g; \cD_f) = 0} ~~\mu(f)
\]
\end{assumption}

\pnote{note in a footnote that we can imagine generalizing to probabilistic distributions by saying "minimal complexity function which samples from $\cD$''}

\begin{assumption}[(weak) Minimal-Description-Length learning]
\label{conj:rasp}
There exists a \emph{complexity measure} on functions $\mu: \mathcal{F} \to \R_{\geq 0}$
such that the following holds.
If a distribution $\cD$ %
admits a perfectly fitting function $f^*$ with small compleixty $\mu(f^*) \leq C$,
and no such function with smaller complexity, then 
The result of training a transformer on $\cD$
is the function $f$.
\end{assumption}

\begin{assumption}[Weak MDL learning (rasp version)]
If a distribution $\cD$
admits a short RASP program $P$ which perfectly fits it,
and no shorter such program,
then training a transformer on $\cD$
will produce a function equivalent to $P$.
\end{assumption}



with the lifted marginals formulation, the question becomes what function is learned by the transformer given the training data.

show that for functions which are simple to learn for a transformer (using rasp as a proxy), the model could naturally and robustly length generalize



We don't claim that RASP is the correct formal way to evaluate this, but it gives good intuition for what functions may be easy to learn by a transformer, since it studies functions that can be easily represented by the attention + mlp mechanism.


\pnote{key point: Length generalization is possible for transformers, because they are defined independent of sequence-length.
By analogy:
We expect RNNs to generalize from short sequences to long ones when both types of sequences are naturally represented by the same RNN. Similarly, we expect Transformers to generalize between two distributions on sequences when both distributions are “naturally represented” by the same transformer. }



==> zoo.tex <==
\section{Zoo of Synthetic Tasks}

Length-generalization in the Counting task is not an isolated phenomenon.
To illustrate the richness and complexity of length-generalization,
we present below a ``zoo'' of synthetic tasks, classified by whether or not they strongly length-generalize.


\begin{figure}[t]
\centering
\includegraphics[width=1.2\textwidth]{figures/add_hinted_lengen.png}
\caption{Length-generalization of Addition, with index-hints (temp figure).
The train distribution is addition of lengths $\in [1, 20]$. The model
is then tested on lengths $+1, +5, +10$ beyond the train length.
Width 512, 8 layers, 6 heads, context length 512.
Median over 16 seeds.
}
\end{figure}

\begin{table}[h!]
    \centering
    \begin{tabular}{p{0.4\linewidth}p{0.4\linewidth}} \toprule
        {\bf Length-Generalizes Well} & {\bf Length-Generalizes Poorly} \\ \midrule
        \noindent
        \begin{itemize}[leftmargin=*]
            \item Counting
            \item Mode
            \item Addition w/ Index Hints, Reversed
            \item Pairity w/ scratchpad, index hints
        \end{itemize} &
        \begin{itemize}[leftmargin=*]
            \item Indexing
            \item Mode with itemized scratchpad
            \item Addition w/ Index Hints, Standard
            \item Pairity without scratchpad
        \end{itemize} \\
        \bottomrule
    \end{tabular}
\end{table}





Our eventual goal is to understand what is different between tasks in the above two sections--- what determines which ones length-generalize?

\pnote{double-check whether relative-position-embeddings affects the story or not.}

\subsection{Discussion: Indexing (and Index Hints)}

\subsection{Experiments}




\begin{table}[t]
\caption{caption}
\label{tab:comp_ke_resnet}
\begin{center}
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{c}{\bf Rasp program}  &\multicolumn{1}{c}{\bf Counterfactual Test}
&\multicolumn{1}{c}{\bf Accuracy}\\ \midrule
Begin with start token &  When the question is presented in reverse order, the model still outputs the start token first& \\
\midrule
If not last token, increment previous token by 1 &  & \\
\midrule
If last token, output EoS & &\\
\bottomrule
\end{tabular}
\end{center}
\end{table}
